On Statistical Rates of Conditional Diffusion Transformers: Approximation, Estimation and Minimax Optimality

We investigate the approximation and estimation rates of conditional diffusion transformers (DiTs) with classifier-free guidance. We present a comprehensive analysis for ``in-context'' conditional DiTs under four common data assumptions. We show that both conditional DiTs and their latent variants lead to the minimax optimality of unconditional DiTs under identified settings. Specifically, we discretize the input domains into infinitesimal grids and then perform a term-by-term Taylor expansion on the conditional diffusion score function under H\"older smooth data assumption. This enables fine-grained use of transformers' universal approximation through a more detailed piecewise constant approximation and hence obtains tighter bounds. Additionally, we extend our analysis to the latent setting under the linear latent subspace assumption. We not only show that latent conditional DiTs achieve lower bounds than conditional DiTs both in approximation and estimation, but also show the minimax optimality of latent unconditional DiTs. Our findings establish statistical limits for conditional and unconditional DiTs, and offer practical guidance toward developing more efficient and accurate DiT models.

==> 5experiments.tex <==


\paragraph{Experimental Objectives.}
We train a conditional diffusion transformer model on the CIFAR10 dataset to validate the following three parts:
\begin{itemize}
    \item \textbf{Objective 1.}
    Validating the influence of input data dimension $d_x$ on the testing loss (score estimation error) in \cref{thm:main_risk_bounds}. 
    \item \textbf{Objective 2.}
    Validating the influence of input data dimension $d_x$ on the parameter norm bounds ($\norm{W_O}_{2,\infty}$ and $\norm{W_V}_{2,\infty}$) in \cref{thm:Main_1}.
    \item \textbf{Objective 3.}
    Validating the influence of backward timestamp $t_0$ on the testing loss (score estimation error) in \cref{thm:main_risk_bounds}.
\end{itemize}



\paragraph{Experimental Details.}
We train the model on the CIFAR10 training dataset for 10 epochs. 
The dataset consists of 50,000 images across 10 classes. 
We set the forward process termination step to $T = 1000$.
Then, we evaluate the model's performance using the CIFAR10 testing dataset of 10,000 images from 10 classes.
We use the testing loss as the measurement. 
\begin{itemize}
    \item 
    To validate objectives 1 and 2, we test various values of $d_x$ at backward timestamp $t_0=5$, including $32 \cdot 32 = 1,024$, $48\cdot 48= 2,304$, $64\cdot 64=4,096$, and $80\cdot 80=6,400$. 

    \item 
    To validate objective 3, we test different backward timestamps $t_0$, including $5, 4, 3, 2$ and $1$ for both $d_x=32\cdot 32=1,024$ and $d_x=48\cdot 48=2,304 $.
\end{itemize}



\paragraph{Model Setup.}
The conditional diffusion transformer model has 12 transformer blocks.
The number of attention heads is $h=6$, and the hidden dimension is $s=384$.
We set the MLP dimension to $r=1536$.
We fix $d=4$ in the DiT reshape layer (\cref{def:reshape_layer}).

\textbf{Computational Resource.}
We conduct all experiments using 1 NVIDIA A100 GPU with 80GB of memory. 
Our code is based on the PyTorch implementation of the diffusion transformer \cite{peebles2023scalable} at \url{https://github.com/chuanyangjin/fast-DiT}.


\subsection{Experimental Results}

\paragraph{Results for Objectives 1 and 2.}
We report the numerical results of  objectives 1 and 2 in \cref{tab:loss_norm_d_x}. 

We observe an increase in the loss value with increasing $d_x$. 
This is consistent with the score estimation result in \cref{thm:main_risk_bounds}.

Additionally, we note an increase in the parameter norm bounds ($\norm{W_O}_{2,\infty}$ and $\norm{W_V}_{2,\infty}$) with increasing $d_x$. 
These align with the parameter norm bound results in \cref{thm:Main_1}.

\begin{table*}[ht]
    \centering
    \caption{{\bf Influence of Input Data Dimension $d_x$ on the Testing Loss and Parameter Norm Bounds at Backward Timestamp $t_0=5$}: The testing loss and parameter norm bounds ($\|W_O\|_{2,\infty}$ and $\|W_V\|_{2,\infty}$) increase with an increasing $d_x$. These results are consistent with the results in \cref{thm:main_risk_bounds} and \cref{thm:Main_1}.}
    \begin{tabular}{@{}l*{4}{c}@{}}
        \toprule
        \text{Input Data Dim.} $d_x$ & $32 \cdot 32 = 1,024$ & $48\cdot 48= 2,304$ & $64\cdot 64=4,096$ & $80\cdot 80=6,400$  \\
        \midrule 
         \text{Testing loss} & 0.9321 & 0.9356 & 0.9364 & 0.9476 \\
        {\bf $\norm{W_O}_{2,\infty}$} & 1.6074 & 1.6332 & 1.6789 & 1.6886  \\
        {\bf $\norm{W_V}_{2,\infty}$} & 2.1513 & 2.1767 & 2.1858 & 2.1994 \\
        \bottomrule
    \end{tabular}
    \label{tab:loss_norm_d_x}
\end{table*}

\paragraph{Results for Objective 3.}
We report numerical results of objectives 3 for $d_x=32 \cdot 32 = 1,024$ and $d_x=48\cdot 48= 2,304$ in \cref{tab:loss_t}.
We observe an increase in the loss value as $t_0$ decreases. 
This is consistent with the score estimation result in \cref{thm:main_risk_bounds}.

\begin{table*}[ht]
    \centering
    \caption{{\bf Influence of Backward Timestamp $t_0$ on the Testing Loss}: The testing loss increases with increasing $t_0$. This is consistent with the result in \cref{thm:main_risk_bounds}.}
    \begin{tabular}{@{}l*{5}{c}@{}}
        \toprule
        \text{Testing loss} & $t_0=5$ & $t_0=4$ & $t_0=3$ & $t_0=2$ & $t_0=1$  
        \\
        \midrule 
        $32 \cdot 32 = 1,024$ & 0.9321 & 0.9329 & 0.9335 & 0.9350 & 0.9361 
        \\
        $48\cdot 48= 2,304$ & 0.9356 & 0.9357 & 0.9360 & 0.9363 & 0.9367 
        \\
        \bottomrule
    \end{tabular}
    \label{tab:loss_t}
\end{table*}


==> boarder.tex <==
To be filled.

